Self-Similarity Among Energy Eigenstates

In a quantum system, different energy eigenstates have different properties or features, allowing us define a classifier to divide them into different groups. We find that the ratio of each type of energy eigenstates in an energy shell $[E_{c}-\Delta E/2,E_{c}+\Delta E/2]$ is invariant with changing width $\Delta E$ or Planck constant $\hbar$ as long as the number of eigenstates in the shell is statistically large enough. We give an argument that such self-similarity in energy eigenstates is a general feature for all quantum systems, which is further illustrated numerically with various quantum systems, including circular billiard, double top model, kicked rotor, and Heisenberg XXZ model.

==> back.tex <==
We discuss the self-similarity with control parameter of $\hbar$ and the energy shell width $\Delta E$ in quantum kicked rotor. 

The self-similarity in the quantum kicked rotor can be examined in two different ways. The first is  the limit of $\hbar_{\textrm{eff}} \sim 0$. 
In Fig.~\ref{fig:selfsim_kr}(a), we show this self-similarity with the classifier
\begin{equation}
    C_{\textrm{width}}(\ket{E}) = \begin{cases}
    1 & W(\ket{E}) > 0.8 \pi \\
    0 & \textrm{otherwise}
    \end{cases}.
    \label{eq:clasf_width}
\end{equation}
The width of Floquet state is defined based on Planck cell basis $\ket{Q,P}$ \cite{otoc}, i.e.,
\begin{equation}
    W(\ket{E})^2 = \sum_{Q, P} \Big[(Q - \pi)^2 + (P-\pi)^2\Big] |\braket{Q,P|E}|^2.
\end{equation}
Geometrically, $W(\ket{E})$ quantifies the ``radius'' of Floquet states to the center point $(q, p) = (\pi, \pi)$. 

The second way of  demonstrating self-similarity is to scale up the width of pseudo-energy shell. Since pseudo-energies are confined into $[0,2\pi)$, original eigenstates with different energies are rearranged into this finite interval. Thus kicked rotor has the same dynamical feature at pseudo-energy shells centered at different pseudo-energy. We emphasize here that this property, i.e., the insensitivity of physics to the center (pseudo-)energy, leads to the consistency between these two approaches to self-similarity. In Fig.~\ref{fig:selfsim_kr})(b), we demonstrate this by checking the entropy of the renormalized distributions of Floquet states in given pseudo-energy shells is roughly independent of the center of the shell. Formally, we compute
\begin{equation}
    p_{Q,P}(E, \Delta E) = \frac {\sum_{E' \in \mathcal{S}(E, \Delta E)} |\braket{Q,P|E'}|^2} {|\mathcal{S}(E, \Delta E)|},
\end{equation}
which is actually the probability distribution $p_{Q,P} = \textrm{Tr}[\ket{Q,P}\bra{Q,P} \hat \rho(E,\Delta E)]$ of maximally mixed state in the energy shell $\hat \rho(E, \Delta E) \propto \sum_{E'\in \mathcal{S}(E,\Delta E)} \ket{E'}\bra{E'}$. Then, we compute the Generalized Wigner-von Neumann entropy (GWvNE)\cite{PhysRevE.99.052117} of it on Planck cell basis (with normalization)
\begin{equation}
    \Gamma(E,\Delta E) = -\frac 1 {\log m^2 }\sum_{Q,P} p_{Q,P}(E,\Delta E) \log p_{Q,P}(E,\Delta E).
    \label{eq:cumu_entropy}
\end{equation}
The function $\log$ is the natural logarithm. By normalization, we make sure $\Gamma \in [0, 1]$. In Fig.~\ref{fig:selfsim_kr}(b), the low variance as center energy $E$ changing demonstrates the independence to $E$ in kicked rotor. Thus, by scaling up the thickness of pseudo-energy shell, more Floquet states are counted and tends to reconstruct the whole phase space. This procedure is similar to our argument about isoenergetic surfaces and is same to our discussion about circular billiard. In Fig.~\ref{fig:selfsim_kr}(c), we show the numerical proof about this result with the classifier by normalized GWvNE of Floquet states, i.e.,
\begin{equation}
    C_{\xi, \textrm{entropy}}(\ket{E}) = \begin{cases}
    1 & S(\ket{E}) \geq \xi \log m^2 \\
    0 & \textrm{otherwise}
    \end{cases},
    \label{eq:clasf_entropy}
\end{equation}
where $S(\ket{E}) = -\sum_{Q,P} \rho_{E;Q,P}\log \rho_{E;Q,P}$ and $\rho_{E;Q,P} = |\braket{Q,P|E}|^2$. We note this classifier is not suitable to study the case of changing $\hbar_{\textrm{eff}}$ since the resolution of phase space varies and the value of entropy (though is normalized) would be dependent of the control parameter $\hbar_{\textrm{eff}}$.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figure/kr_selfsim.pdf}
    \caption{
    The self-similarity of two aspects in kicked rotor. (a) the ratio by classifier defined in Eq.~\ref{eq:clasf_width} to the reciprocal of effective Planck constant. (b) the cumulated entropy $\Gamma(E,\Delta E)$ defined by Eq.~\ref{eq:cumu_entropy} to the center pseudo-energy $E$. The pseudo-energy shell width $\Delta E = 0.4$ here. (c) the ratio by classifier defined in Eq.~\ref{eq:clasf_entropy} to the pseudo-energy shell width $\Delta E$. The center pseudo-energy $E=0$ and the factor $\xi = 0.6$ for $K=1.1$ and $40\times 40$ Planck cells. (d) the number of Floquet states within the pseudo-energy shell considered in $(c)$.}
    \label{fig:selfsim_kr}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{figure/XXZ_selfsimilar.pdf}
    \caption{The ratio $f$ for various classifiers: (a)magnetization for a single spin (6th-spin), (b)total magnetization, (c)two-spin-correlation for 3rd spin and 4th spin, (d)global-X-correlation, (e)2nd R\'enyi entropy of 1st spin. (f) shows the total number of energy eigenstates in energy shell $[E_{c}-\Delta E/2,E_{c}+\Delta E/2]$. We take the length of spin chain to be $N=12$, parameter $\rho=0.4$ and central energy $E_{c}=4$.}
    \label{fig:XXZ}
\end{figure*}

==> self_similarity_arxiv(v1)/back.tex <==
We discuss the self-similarity with control parameter of $\hbar$ and the energy shell width $\Delta E$ in quantum kicked rotor. 

The self-similarity in the quantum kicked rotor can be examined in two different ways. The first is  the limit of $\hbar_{\textrm{eff}} \sim 0$. 
In Fig.~\ref{fig:selfsim_kr}(a), we show this self-similarity with the classifier
\begin{equation}
    C_{\textrm{width}}(\ket{E}) = \begin{cases}
    1 & W(\ket{E}) > 0.8 \pi \\
    0 & \textrm{otherwise}
    \end{cases}.
    \label{eq:clasf_width}
\end{equation}
The width of Floquet state is defined based on Planck cell basis $\ket{Q,P}$ \cite{otoc}, i.e.,
\begin{equation}
    W(\ket{E})^2 = \sum_{Q, P} \Big[(Q - \pi)^2 + (P-\pi)^2\Big] |\braket{Q,P|E}|^2.
\end{equation}
Geometrically, $W(\ket{E})$ quantifies the ``radius'' of Floquet states to the center point $(q, p) = (\pi, \pi)$. 

The second way of  demonstrating self-similarity is to scale up the width of pseudo-energy shell. Since pseudo-energies are confined into $[0,2\pi)$, original eigenstates with different energies are rearranged into this finite interval. Thus kicked rotor has the same dynamical feature at pseudo-energy shells centered at different pseudo-energy. We emphasize here that this property, i.e., the insensitivity of physics to the center (pseudo-)energy, leads to the consistency between these two approaches to self-similarity. In Fig.~\ref{fig:selfsim_kr})(b), we demonstrate this by checking the entropy of the renormalized distributions of Floquet states in given pseudo-energy shells is roughly independent of the center of the shell. Formally, we compute
\begin{equation}
    p_{Q,P}(E, \Delta E) = \frac {\sum_{E' \in \mathcal{S}(E, \Delta E)} |\braket{Q,P|E'}|^2} {|\mathcal{S}(E, \Delta E)|},
\end{equation}
which is actually the probability distribution $p_{Q,P} = \textrm{Tr}[\ket{Q,P}\bra{Q,P} \hat \rho(E,\Delta E)]$ of maximally mixed state in the energy shell $\hat \rho(E, \Delta E) \propto \sum_{E'\in \mathcal{S}(E,\Delta E)} \ket{E'}\bra{E'}$. Then, we compute the Generalized Wigner-von Neumann entropy (GWvNE)\cite{PhysRevE.99.052117} of it on Planck cell basis (with normalization)
\begin{equation}
    \Gamma(E,\Delta E) = -\frac 1 {\log m^2 }\sum_{Q,P} p_{Q,P}(E,\Delta E) \log p_{Q,P}(E,\Delta E).
    \label{eq:cumu_entropy}
\end{equation}
The function $\log$ is the natural logarithm. By normalization, we make sure $\Gamma \in [0, 1]$. In Fig.~\ref{fig:selfsim_kr}(b), the low variance as center energy $E$ changing demonstrates the independence to $E$ in kicked rotor. Thus, by scaling up the thickness of pseudo-energy shell, more Floquet states are counted and tends to reconstruct the whole phase space. This procedure is similar to our argument about isoenergetic surfaces and is same to our discussion about circular billiard. In Fig.~\ref{fig:selfsim_kr}(c), we show the numerical proof about this result with the classifier by normalized GWvNE of Floquet states, i.e.,
\begin{equation}
    C_{\xi, \textrm{entropy}}(\ket{E}) = \begin{cases}
    1 & S(\ket{E}) \geq \xi \log m^2 \\
    0 & \textrm{otherwise}
    \end{cases},
    \label{eq:clasf_entropy}
\end{equation}
where $S(\ket{E}) = -\sum_{Q,P} \rho_{E;Q,P}\log \rho_{E;Q,P}$ and $\rho_{E;Q,P} = |\braket{Q,P|E}|^2$. We note this classifier is not suitable to study the case of changing $\hbar_{\textrm{eff}}$ since the resolution of phase space varies and the value of entropy (though is normalized) would be dependent of the control parameter $\hbar_{\textrm{eff}}$.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figure/kr_selfsim.pdf}
    \caption{
    The self-similarity of two aspects in kicked rotor. (a) the ratio by classifier defined in Eq.~\ref{eq:clasf_width} to the reciprocal of effective Planck constant. (b) the cumulated entropy $\Gamma(E,\Delta E)$ defined by Eq.~\ref{eq:cumu_entropy} to the center pseudo-energy $E$. The pseudo-energy shell width $\Delta E = 0.4$ here. (c) the ratio by classifier defined in Eq.~\ref{eq:clasf_entropy} to the pseudo-energy shell width $\Delta E$. The center pseudo-energy $E=0$ and the factor $\xi = 0.6$ for $K=1.1$ and $40\times 40$ Planck cells. (d) the number of Floquet states within the pseudo-energy shell considered in $(c)$.}
    \label{fig:selfsim_kr}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{figure/XXZ_selfsimilar.pdf}
    \caption{The ratio $f$ for various classifiers: (a)magnetization for a single spin (6th-spin), (b)total magnetization, (c)two-spin-correlation for 3rd spin and 4th spin, (d)global-X-correlation, (e)2nd R\'enyi entropy of 1st spin. (f) shows the total number of energy eigenstates in energy shell $[E_{c}-\Delta E/2,E_{c}+\Delta E/2]$. We take the length of spin chain to be $N=12$, parameter $\rho=0.4$ and central energy $E_{c}=4$.}
    \label{fig:XXZ}
\end{figure*}
